MD-Bench: Engineering the in-core performance of short-range molecular dynamics kernels from state-of-the-art simulation packages

Molecular dynamics (MD) simulations provide considerable benefits for the investigation and experimentation of systems at atomic level. Their usage is widespread into several research fields, but their system size and timescale are also crucially limited by the computing power they can make use of. Performance engineering of MD kernels is therefore important to understand their bottlenecks and point out possible improvements. For that reason, we developed MD-Bench, a proxy-app for short-range MD kernels that implements state-of-the-art algorithms from multiple production applications such as LAMMPS and GROMACS. MD-Bench is intended to have simpler, understandable and extensible source code, as well as to be transparent and suitable for teaching, benchmarking and researching MD algorithms. In this paper we introduce MD-Bench, describe its design and structure and implemented algorithms. Finally, we show five usage examples of MD-Bench and describe how these are useful to have a deeper understanding of MD kernels from a performance point of view, also exposing some interesting performance insights.

==> doc/tmp.tex <==
....
....

\end{abstract}

%%Graphical abstract
\begin{graphicalabstract}
%\includegraphics{grabs}
\end{graphicalabstract}

%%Research highlights
\begin{highlights}
\item Research highlight 1
\item Research highlight 2
\end{highlights}

\begin{keyword}
%% keywords here, in the form: keyword \sep keyword
....
....

